Counting Defective Parking Functions

Suppose that $n$ drivers each choose a preferred parking space in a linear car park with $m$ spaces. Each driver goes to the chosen space and parks there if it is free, and otherwise takes the first available space with larger number (if any). If all drivers park successfully, the sequence of choices is called a parking function. In general, if $k$ drivers fail to park, we have a \emph{defective parking function} of \emph{defect} $k$. Let $\cp(n,m,k)$ be the number of such functions. In this paper, we establish a recurrence relation for the numbers $\cp(n,m,k)$, and express this as an equation for a three-variable generating function. We solve this equation using the kernel method, and extract the coefficients explicitly: it turns out that the cumulative totals are partial sums in Abel's binomial identity. Finally, we compute the asymptotics of $\cp(n,m,k)$. In particular, for the case $m=n$, if choices are made independently at random, the limiting distribution of the defect (the number of drivers who fail to park), scaled by the square root of $n$, is the Rayleigh distribution. On the other hand, in case $m=\omega(n)$, the probability that all spaces are occupied tends asymptotically to one.

==> Makefile <==
MASTER      = Carpark_CameronJohannsenPrellbergSchweitzer
# Name of .pstex-files to be generated (with .pstex)
#GRAPHICS    = image.pstex
# Scale xfig-Images by this value
SCALEFIG = 0.75
# Paper size for dvips/ps2pdf
PAPER = a4
# Set to 1 if xtimes should be run
XTIMES = 0

.SUFFIXES: dvi ps pdf pstex pstex_t

CLEAN_FILES = *.aux *.log *.pdf *.bbl *.blg tmp.* *.pstex *.pstex_t *.out $(MASTER).dvi $(MASTER).ps $(MASTER).pdf *~
TEXSOURCES = *.tex

all: clean pdf

# for latex
%.dvi: %.tex $(GRAPHICS) $(TEXSOURCES) # %.bib
	rm -rf tmp.*
ifeq ($(XTIMES),1)
	bash xtimes
endif
	latex $<
	( grep citat $(*F).aux >/dev/null && bibtex $(*F) ) || true
	latex $<
	echo "Final latex run.."
	latex $<
	rm -rf tmp.who tmp.unsorted tmp.sorted tmp.date

%.ps: %.dvi
	dvips -Ppdf -t$(PAPER) $<
#	dvips -Ppdf $<
#       -ups will work on all mpi-machines and probably gives better .pdf

%.pdf: %.ps
	ps2pdf14 -dPDFSETTINGS=/printer -dMaxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=$(PAPER) -dUseCIEColor=true $<

%.pstex: %.fig
	fig2dev -Lpstex -m $(SCALEFIG) -n $@ $< $@
	fig2dev -Lpstex_t -p $(*F).pstex -m $(SCALEFIG) $< $@_t

%.pstex_t: %.fig
	fig2dev -Lpstex_t -p $(*F).pstex -m $(SCALEFIG) $< $@


# high level (PHONY) rules for convenience
latex dvi: $(MASTER).dvi

ps postscript dvips: $(MASTER).ps

pdf: $(MASTER).pdf

warnings:
	latex $(MASTER).tex | grep "Warning"

clean:
	rm -f $(CLEAN_FILES)

add:
	for i in *.tex; \
	do \
	  if ( ! head -1 $$i | grep "%$$Date" ) >/dev/null ; then \
	    (echo -e "% \$$Date$$\n% \$$Revision$$\n% \$$Author$$" ; cat $$i) > $$i.tmp; \
	    mv $$i.tmp $$i ; \
	    svn add $$i ; \
	    svn propset svn:keywords "Date Rev Author" $$i ; \
	  fi; \
	done

keywords:
	svn propset svn:keywords "Date Rev Author" *.tex

.PHONY: pdf dvi latex ps postscript dvips view clean

